Multiple Resource Allocation in Multi-Tenant Edge Computing via Sub-modular Optimization

Edge Computing (EC) allows users to access computing resources at the network frontier, which paves the way for deploying delay-sensitive applications such as Mobile Augmented Reality (MAR). Under the EC paradigm, MAR users connect to the EC server, open sessions and send continuously frames to be processed. The EC server sends back virtual information to enhance the human perception of the world by merging it with the real environment. Resource allocation arises as a critical challenge when several MAR Service Providers (SPs) compete for limited resources at the edge of the network. In this paper, we consider EC in a multi-tenant environment where the resource owner, i.e., the Network Operator (NO), virtualizes the resources and lets SPs run their services using the allocated slice of resources. Indeed, for MAR applications, we focus on two specific resources: CPU and RAM, deployed in some edge node, e.g., a central office. We study the decision of the NO about how to partition these resources among several SPs. We model the arrival and service dynamics of users belonging to different SPs using Erlang queuing model and show that under perfect information, the interaction between the NO and SPs can be formulated as a sub-modular maximization problem under multiple Knapsack constraints. To solve the problem, we use an approximation algorithm, guaranteeing a bounded gap with respect to the optimal theoretical solution. Our numerical results show that the proposed algorithm outperforms baseline proportional allocation in terms of the number of sessions accommodated at the edge for each SP.

==> draft.tex <==
\subsection{Related work from external paper}
This related work is taken from a paper ``Road to 6g'' about cost in 6G Andrea reviewed for IFIP 2022. We should read the papers cited here and add them in our literature review

3GPP TR 22.852 proposes an on-demand automated
Capacity Broker for RAN resources [8]. K. Samdanis et al.
move one step forward and introduce the 5G Network Slice
Broker concept. It offers slices to shared network tenants via
3GPP Service Capacity Exposure Function (SCEF) [9].
Infrastructure sharing also comes up at [10], where Xin Li et
al. talk about resource sharing in 5G in general and list the
upcoming challenges. One of their publications is "Network
Store" by Navid Nikaein et al. [11], a digital distribution
platform of programmable Virtual Network Functions. It is a
digital marketplace of Network Application and Functions
on the top of commodity cloud infrastructures on the fly.
Balazs Gero et al. [12] within the 5Gex consortium [13]
deal with cross-domain orchestration where a 3 rd party
olution provider offers telecommunication services (Virtual
Network Function as a Service, VNFaaS) in a multi-provider
5G environment. Özgür Umut Akgül et al. [14] propose a
platform for dynamic network slice sharing and trading for
tenants on the same underlying infrastructure.
Cloud Stock Exchange (CSE) concept is introduced for
inter-provider resource sharing [5] [15] [16]. It shows a
possible way for both infrastructure sharing and its
accounting and charging, using assets from the financial
industry. It envisions a stock-exchange market-like resource
trading which may by applicable for telecommunication
resource management. with spot [17], future [18] and option
markets [19].
TCO calculations for 5G networks have already been
proposed. Wolfgang Kiess et al. [20] examine the TCO of 5G
services, where the TCO model considers the following
factors: datacenter CAPEX and OPEX, IT hardware CAPEX
and OPEX, IT administration OPEX and Network Element
(NE) CAPEX. They calculate NE administration cost (NE
OPEX) on operator network level based on the number of
NE instances used in all data centers and assume NE
administration to be done remotely from operation support
center(s). They consider deployments' cost too. In the end,
relative costs are presented for each type of service. Jozsef
Varga et al. [21] present calculations to reduce OPEX for
Ultra-Reliable Low-Latency (uRLL) services. They prove
that infrastructure sharing is a way to decrease OPEX, but it
is geographically limited. Juhon Kim et al. [22] talk about a
roaming scenario in which (home) telecommunication
infrastructure of roaming users is instantiated at the visited
network. E.g., a virtual Packet Gateway (vPGW) is set up in
the foreign network to serve the users' needs.

REFERENCES

 [1] S. Nayak and R. Patgiri, ‘6G Communication: Envisioning the Key
Issues and Challenges’, EAI Endorsed Transactions on Internet of
Things, vol. 6, p. 166959, Nov. 2020, doi: 10.4108/eai.11-11-
2020.166959.
[2] K. Sheth, K. Patel, H. Shah, S. Tanwar, R. Gupta, and N. Kumar, ‘A
Taxonomy of AI Techniques for 6G Communication Networks’,
Computer Communications, vol. 161, Jul. 2020, doi:
10.1016/j.comcom.2020.07.035.
[3] W. Saad, M. Bennis, and M. Chen, ‘A Vision of 6G Wireless
Systems: Applications, Trends, Technologies, and Open Research
Problems’, IEEE Network, vol. 34, no. 3, pp. 134–142, 2020, doi:
10.1109/MNET.001.1900287.
[4] McKinsey, ‘Network sharing and 5G: A turning point for lone
riders’. https://www.mckinsey.com/industries/technology-media-and-
telecommunications/our-insights/network-sharing-and-5g-a-turning-
point-for-lone-riders (accessed Sep. 15, 2021).
[5] A. Leiter, ‘Cloud Stock Exchange for Telecommunication’, in 2018
International Symposium on Networks, Computers and
Communications (ISNCC), 2018, pp. 1–4. doi:
10.1109/ISNCC.2018.8531052.
[6] ‘Digital Single Market - Roaming’. https://ec.europa.eu/digital-
single-market/en/roaming (accessed Sep. 15, 2021).
[7] ‘International Roaming BEREC Benchmark Data Report October
2017 - March 2018’.
https://berec.europa.eu/eng/document_register/subject_matter/berec/r
eports/8251-international-roaming-berec-benchmark-data-report-
october-2017-march-2018 (accessed Sep. 15, 2021).
[8] ‘3GPP - TR 22.852: Study on Radio Access Network (RAN) sharing
enhancements’.
https://portal.3gpp.org/desktopmodules/Specifications/SpecificationD
etails.aspx?specificationId=668 (accessed Sep. 15, 2021).
[9] K. Samdanis, X. Costa-Pérez, and V. Sciancalepore, ‘From Network
Sharing to Multi-tenancy: The 5G Network Slice Broker’, IEEE
Communications Magazine, vol. 54, Jul. 2016, doi:
10.1109/MCOM.2016.7514161.
[10] X. Li et al., ‘Network Slicing for 5G: Challenges and Opportunities’,
IEEE Internet Computing, vol. PP, pp. 1–1, Aug. 2018, doi:
10.1109/MIC.2018.326150452.
[11] N. Nikaein et al., ‘Network Store: Exploring Slicing in Future 5G
Networks’, in Proceedings of the 10th International Workshop on
Mobility in the Evolving Internet Architecture, New York, NY, USA,
2015, pp. 8–13. doi: 10.1145/2795381.2795390.
[12] B. Gerő et al., ‘The orchestration in 5G exchange — A multi-
provider NFV framework for 5G services’, in 2017 IEEE Conference
on Network Function Virtualization and Software Defined Networks
(NFV-SDN), 2017, pp. 1–2. doi: 10.1109/NFV-SDN.2017.8169865.
[13] ‘5Gex project’. https://5g-ppp.eu/5gex/ (accessed Sep. 15, 2021).
[14] Ö. U. Akgül, I. Malanchini, and A. Capone, ‘Dynamic Resource
Trading in Sliced Mobile Networks’, IEEE Transactions on Network
and Service Management, vol. 16, no. 1, pp. 220–233, 2019, doi:
10.1109/TNSM.2019.2893126.
[15] Á. Leiter and L. Bokor, ‘Stock market trading strategies and cost
estimation for telecommunication resource management’, in 2019
10th International Conference on Networks of the Future (NoF),
2019, pp. 126–129. doi: 10.1109/NoF47743.2019.9015018.
[16] Á. Leiter and L. Bokor, ‘A Study on Use Cases and Business Aspects
of Cloud Stock Exchange’, in 2020 International Conference on
Information Networking (ICOIN), 2020, pp. 732–737. doi:
10.1109/ICOIN48656.2020.9016536.
[17] ‘Spot market’. https://www.investopedia.com/terms/s/spotmarket.asp
(accessed Sep. 15, 2021).
[18] ‘Futures market’.
https://www.investopedia.com/terms/f/futurescontract.asp (accessed
Sep. 15, 2021).
[19] ‘Options market’. https://www.investopedia.com/terms/o/option.asp
(accessed Sep. 15, 2021).
[20] W. Kiess, M. R. Sama, J. Varga, J. Prade, H.-J. Morper, and K.
Hoffmann, ‘5G via evolved packet core slices: Costs and technology
of early deployments’, in 2017 IEEE 28th Annual International
Symposium on Personal, Indoor, and Mobile Radio Communications
(PIMRC), 2017, pp. 1–7. doi: 10.1109/PIMRC.2017.8292691.
[21] J. Varga, A. Hilt, J. Bíró, C. Rotter, and G. Jaro, ‘Reducing
operational costs of ultra-reliable low latency services in 5G’,
Infocommunications Journal, vol. X, pp. 37–45, 2018, doi:
10.36244/ICJ.2018.4.6.
[22] J. Kim et al., ‘GiLAN Roaming: Roam Like at Home in a Multi-
Provider NFV Environment’, in 2018 International Symposium on
Networks, Computers and Communications (ISNCC), 2018, pp. 1–4.
doi: 10.1109/ISNCC.2018.8530973.
[23] ‘International Roaming BEREC Benchmark Data Report October
2019 – March 2020’.
https://berec.europa.eu/eng/document_register/subject_matter/berec/r
eports/9443-international-roaming-berec-benchmark-data-report-
october-2019-march-2020-2nd-western-balkan-roaming-report
(accessed Sep. 16, 2021).
[24] V. Valancius, C. Lumezanu, N. Feamster, R. Johari, and V. V.
Vazirani, ‘How Many Tiers? Pricing in the Internet Transit Market’,
SIGCOMM Comput. Commun. Rev., vol. 41, no. 4, pp. 194–205,
Aug. 2011, doi: 10.1145/2043164.2018459.
[25] ‘Amazon Spot Market’. https://aws.amazon.com/de/ec2/spot/
(accessed Sep. 17, 2021).
[26] D. Reddy and V. Clinton, ‘Simulating stock prices using geometric
Brownian motion: Evidence from Australian companies’, vol. 10, pp.
23–47, Jan. 2016, doi: 10.14453/aabfj.v10i3.3.
[27] K. Suganthi and G. Jayalalitha, ‘Geometric Brownian Motion in
Stock Prices’, Journal of Physics: Conference Series, vol. 1377, p.
012016, Nov. 2019, doi: 10.1088/1742-6596/1377/1/012016.
[28] M. Mohd Jaffar and S. Zainol Abidin, ‘Forecasting Share Prices of
Small Size Companies in Bursa Malaysia Using Geometric Brownian
Motion’, Applied Mathematics & Information Sciences, vol. 6, Dec.
2012.
[29] W. F. Agustini, I. R. Affianti, and E. R. Putri, ‘Stock price prediction
using geometric Brownian motion’, Journal of Physics: Conference
Series, vol. 974, p. 012047, Mar. 2018, doi: 10.1088/1742-
6596/974/1/012047.
[30] P. Hegyi, N. Varga, and L. Bokor, ‘An advanced telco cloud
simulator and its usage on modelling multi-cloud and 5G multi-
access environments’, in 2018 21st Conference on Innovation in
Clouds, Internet and Networks and Workshops (ICIN), Feb. 2018, pp.
1–3. doi: 10.1109/ICIN.2018.8401637.
[31] P. Hegyi and J. Varga, ‘Telco Cloud Simulator’, in 2019 IEEE 24th
International Workshop on Computer Aided Modeling and Design of
Communication Links and Networks (CAMAD), 2019, pp. 1–7. doi:
10.1109/CAMAD.2019.8858483.
[32] D. Madan and Y. Xiao, ‘Leveraged Levy processes as models for
stock prices’, Quantitative Finance, vol. 10, pp. 735–748, Aug. 2010,
doi: 10.1080/14697680903067138.
[33] W. Arowolo, ‘Predicting Stock Prices Returns Using Garch Model’,
2013.
[34] N. Thai Hung, ‘An empirical analysis on volatility: Evidence for the
Budapest stock exchange using Garch model’, Journal of
Development and Integration, Jan. 2017.





%%%%%%%%%%%%%%%%%% figure %%%%%%%%%%%%%%%%%%%%%

\begin{figure}
    \centering
    \begin{tikzpicture}[node distance = 2cm, auto]
    % Place nodes
    \node [point] (start) {Start};
    \node [decision, below of=start, node distance=2.5cm] (dec2) {$T_r^{\text{c}} \textless \tau_r$};
    \node [decision, right of=dec2, node distance=2.5cm] (dec1){$T_r^{\text{e}} \textless \tau_r$};
    \node [block, right of=dec1, node distance=2.5cm] (lost) {Lost};
    \node [block, below of=dec1, node distance=3cm] (edge) {Edge};
    \node [block, below of=dec2, node distance=3cm] (cloud) {Cloud};
    \node [point, below of=cloud, node distance=3cm] (end) {End};

    
    % Draw edges
    \path [line] (start) -- (dec2);
    \path [line] (dec2) -- node {yes} (cloud);
    \path [line] (dec2) -- node {no}(dec1);
    \path [line] (dec1) -- node {yes}(edge);
    \path [line] (dec1) -- node {no}(lost);
    \path [line] (edge) -- (end);
    \path [line] (cloud) -- (end);
    \path [line] (lost) -- ++(2,0) |- (end);

    \end{tikzpicture}
    \caption{SP Decision Process}
    \label{fig:sp-desicion-process}
\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Mathematical Model}

Let us denote the set of requests coming from SP $p$ at a time slot $t$ by $\mathcal{R}^t_p$: 
\begin{align}
    \mathcal{R}^t_p = \{r = (\tau_r, \sigma^{\text{data}}_r, \sigma^{\text{CPU}}_r, \$_r^{\text{edge}}, \$_r^{\text{cloud}}) \}
\end{align}

Our goal is to serve a request $r \in \mathcal{R}^t_p$ in the edge node such that its total serving time $T_r$ is less than the tolerance delay $\tau_r$, which represents the maximum time of treating that request $r$.
The total serving time $T_r$ is the sum of:

\textbf{(1) Wireless Network Latency:} The wireless network latency for transmitting the user traffic for SP $p$, denoted by $T^{\text{W}}_p$, can be computed as:
\begin{align}
\label{eq:processing-latency}
    T^{\text{W}}_r = \frac{\sigma^{\text{data}}_r}{\beta_p^{\text{W}} \cdot C^{\text{W}}}
\end{align}
where $\sigma^{\text{data}}$ is the size of data transmitted in the request and $\beta_p^{\text{W}} \cdot C^{\text{W}}$ is the capacity of the network slice for SP $p$ in the edge network. The following constraints ensure that the capacity of all slices does not exceed the total capacity $C^{\text{W}}$ of the edge network, and $\beta_p^{\text{W}} \cdot C^{\text{W}}$ is higher than the corresponding $\lambda_p$:
\begin{align}
\label{eq:contraints-1}
    \sum_{p = 1}^{P} \beta_p^{\text{W}}  \leq 1 \\
    \lambda_p \textless \beta_p^{\text{W}} \cdot C^{\text{W}}, \forall p \in [1,P]
\end{align}

\textbf{(2) Processing Latency:} We assume that each SP request can be processed on one edge node, and the edge node can slice its computation capacity to serve different SPs.
Let $T^{\text{CPU}}_p$ denote the processing latency of a request to SP $p$. Then, based on the computational capacity slice and the amount of traffic served on the edge node, the processing latency $T^{\text{CPU}}_p$, $p~=~1,~\dots,~P$, is expressed as follows:
\begin{align}
    T^{\text{CPU}}_r = \frac{\sigma^{\text{CPU}}_r}{\beta_p^{\text{CPU}} \cdot C^{\text{CPU}}}
\label{eq:processing-latency}
\end{align}
where $\sigma^{\text{CPU}}$ is the size of the request (i.e. the number of instructions) and $\beta_p^{\text{CPU}} \cdot C^{\text{CPU}}$ is the capacity of the CPU slice for SP $p$. In the above equation, $\beta_p^{\text{CPU}}$ has to fulfill the consistency constraint:
\begin{align}
\label{eq:contraints-3}
    \sum_{p = 1}^{P} \beta_p^{\text{CPU}}  \leq 1 
\end{align}

\textbf{(3) Queuing Latency:} We assume that each request is stacked in a queue until it can be sent and then in another queue until it can be executed.
\begin{align}
    T^{\text{Q, CPU}}_r = \frac{1}{\mu_p - \lambda^{\text{edge}}_p} - \frac{1}{\mu_p}
\label{eq:queue-latency}
\end{align}
where $\frac{1}{\mu_p}$ is the processing time defined by~(\ref{eq:processing-latency}).

Therefore, the total serving time $T_r$ can be written as follows: 
\begin{align}
    T_r^e = T_r^W + T_r^{\text{CPU,e}} + T_r^{\text{Q, CPU}}\\
        = \frac{\sigma^{\text{data}}_r}{\beta_p^{\text{W}} \cdot C^{\text{W}}} 
        + \frac{\sigma^{\text{CPU}}_r}{\beta_p^{\text{CPU}} \cdot C^{\text{CPU}}}
        + \frac{1}{\mu_p - \lambda_p} - \frac{1}{\mu_p}\\
        = \frac{\sigma^{\text{data}}_r}{\beta_p^{\text{W}} \cdot C^{\text{W}}} 
        + \frac{1}{\mu_p - \lambda_p}\\
        = \frac{\sigma^{\text{data}}_r}{\beta_p^{\text{W}} \cdot C^{\text{W}}} 
        + \frac{\sigma^{\text{CPU}}_r}{\beta_p^{\text{CPU}} \cdot C^{\text{CPU}} - \sigma^{\text{CPU}}_r \cdot \lambda_p} 
\label{eq:total-serving-time}
\end{align}

\todoi{Write $T_r^e$ and $T_r^c$, i.e., the time to complete the request (transmission, queueing processing) in the edge or in the cloud, respectively.}

For any request $r$ of SP $p$ going to the cloud server, we have an extra latency that represents the time it takes to transmit the request from the edge node to the origin cloud sever of SP $p$, which we denote by $T_r^{e,c}$.
We suppose that there is enough processors in the cloud server, thus we do not consider $T^{\text{Q, CPU}}_r$. (see \url{https://blog.scaleway.com/understanding-network-latency/}).
Therefore, the total serving time for a request $r$ served in the cloud server can be written as follows:
\begin{align}
    T_r^c = T_r^W + T_r^{e,c} + T_r^{\text{CPU,c}}
\end{align}


 
\subsection{Optimization Problem}
\todoi{aa: lambda price. Write a reference}
The NO objective is to maximize its profits by maximizing the number of requests executed on the edge, since the SP pays for each request processed on the edge node.
\begin{align}
    \$_r^{\text{edge}} = g(\sigma_r^{\text{CPU}}, \sigma_r^{\text{data}})
\end{align}

For a request $r\in\mathcal{R}_p^t$
\begin{align}
    \text{rev}_r (\beta_p^W, \beta_p^{\text{CPU}}) 
    &:= 
    \mathbbm{1} \{ \alpha_r^{\text{edge}} = 1 \} \tag{$\CMcal{P}0$} \cdot \$_r^{\text{edge}}\\
    &= \mathbbm{1} \{ T_r^c > \tau_r \text{ and } T_r^e < \tau_r \}\cdot \$_r^{\text{edge}}\\
    & =\mathbbm{1} \{ T_r^c > \tau_r \}\cdot \mathbbm{1} \{ T_r^e < \tau_r \}\cdot \$_r^{\text{edge}}
\end{align}

We now denote the expected value of the revenue of any request of SP $p$ as:
\begin{align}
    \mathbb{E}\text{rev}_r (\beta_p^W, \beta_p^{\text{CPU}}) 
    & =\mathbb{P} \{ T_r^c > \tau_r \}\cdot \mathbb{P} \{ T_r^e < \tau_r \}\cdot \mathbb{E}\$_r^{\text{edge}}
\end{align}

\begin{align}
    \mathbb{E}\text{rev}_p (\beta_p^W, \beta_p^{\text{CPU}}) 
    &:= 
    \mathbb{E} R_p\cdot \mathbb{E}\text{rev}_r (\beta_p^W, \beta_p^{\text{CPU}})
\end{align}
where $\mathbb{E}R_p$ is the expected amount of requests for SP $p$ in a timeslot.
\begin{align}
    \mathbb{E}\text{rev} (\vec\beta^W, \vec\beta^{\text{CPU}}) 
    &:= 
    \sum_{p=1}^P \mathbb{E}\text{rev}_p (\beta_p^W, \beta_p^{\text{CPU}}) 
\end{align}

\todoi{aa: Is the function we want to optimize continuous/concave w.r.t. our betas. To show it, it suffices to show that $\mathbb{P} \{ T_r^e < \tau_r \}$ is continuous/concave w.r.t. $\beta_p^W, \beta_p^{\text{CPU}}$?}

The optimization can be written, from the NO perspective, as:
\begin{align}
    \max_{\vec\beta^{\text{W}}, \vect\beta^{\text{CPU}}}
    \mathbb{E}\text{rev} (\vec\beta^W, \vec\beta^{\text{CPU}}) 
\label{eq:opt-problem-NO}
\end{align}
where:
\begin{align}
\label{eq:alpha-function}
    \alpha_r^{\text{edge}} 
    &= 
    \begin{cases}
			1, & \text{if $r$ is processed on the edge node}\\
            0, & \text{otherwise}
	\end{cases}\\
    &=\begin{cases}
			1, & \text{if $T_r^e<\tau_r \text{ and } \$_r^e < \$_r^c$}\\
            0, & \text{otherwise}
	\end{cases}
\end{align} 


==> old-parts/2023-01-23.tex <==
- Why do we use the streaming algorithm? Computing the optimal value has scalability problems?
- Let's add the wifi-5G-resource block in the resource pool (we thus have 3 resource types), otherwise we are actually only allocating CPU
- Let's plot actual average delay instead of f.
- We cannot simply use formulation of [1] as multiple resources are more complicated.
[1] Chu, W., Dehghan, M., Lui, J. C. S., Towsley, D., & Zhang, Z. L. (2018). Joint cache resource allocation and request routing for in-network caching services. Computer Networks, 131, 1–14. https://doi.org/10.1016/j.comnet.2017.11.009

==> old-parts/multidimensional-knapsack.tex <==
%%%%%%%%%%%%%% D KNAPSACK PROBLEM %%%%%%%%%%%%%%%%%%%
\section{Multidimensional Knapsack Formulation}
\label{sec:multi-knapsack-formulation}

Problem~\eqref{eq:opt-prob-2} can be seen as a general Multi-Dimensional Knapsack Problem (MDKP)~\cite{akccay2007} with $d~=~|\mathcal{R}|$ dimensions, with the capacity of the each dimension being $K^r$, $r \in \mathcal{R}$. There are P different items and let $n_p$ be the number of copies of item $p$, $p = 1 \dots P$. The $p$-th item requires $z_p^r$ units of the dimension $r$ of the knapsack.
The capacity constraint in~\eqref{eq:opt-prob-2} is thus satisfied if and only if we select $n_p$ number of copies for $p=1,\dots,P$ such that $z_p\cdot n_p\le K^r,\forall r \in\mathcal{R}$.
The reward of including a single copy of item $p$ in the knapsack is $w_p$. The objective is to maximize the total reward of the selected items.

Our problem can be seen as a Multi-Dimensional Knapsack Problem (MDKP) with a collection of different resource constraints. The number of resources $d~=~|\mathcal{R}|$ is the dimensions of the knapsack. The number of SPs is the number of items and the number of copies of each item is the maximum number of users for each SP. The requirement of one single user of SP $p$ in terms of resource $r$ is $z_p^r$.

Therefore, we can formulate our problem as follows:

\begin{equation}
\begin{aligned}
    \text{maximize} \quad & \sum_{p=1}^P w_p n_p\\
    \textrm{s.t.} \quad & \sum_{p=1}^P z_p^r n_p \leq K^r,  \forall r\in\mathcal{R}\\
    & n_p \in \mathbb{N}
\label{eq:opt-prob-multi-dim-knap-prob}
\end{aligned}
\end{equation}

When the decision variables are constrained to be binary variables $n_p \in \{0, 1\}, p = 1 \dots P$, the above problem is commonly referred to as the 0-1 MDKP. Since in our case $n_p\in\mathbb{N}$, our problem is a general MDKP. Both the 0-1 MDKP and general MDKP are \emph{strongly} NP-hard~\cite{garey1979}. 
Unlike the extensive researches that have been conducted for the 0-1 MDKP, the solution approaches for the general MDKP are scarce. %Generalizations of the approximate solution methods intended for the 0-1 MDKP fail to yield efficient solutions for the general MDKP, unless the number of resource constraints or the upper bounds of the decision variables is small~\cite{lin1998}.
%\todo{aa: In our case, are they small or big? Motivate this.}

\begin{comment}
    

Similar to us, authors of~\cite{akccay2007} aim to solve (\ref{eq:opt-prob-multi-dim-knap-prob}). They propose a greedy-like heuristic method based on the notion of \emph{effective capacity}, which is by definition, $\min_r\{\frac{\bar{K^r}}{z^r_p}\}$, where $\bar{K^r}$ is the the remaining capacity of resource $r$. The \emph{effective capacity} is intuitively understood as the maximum
number of users of SP $p$ that can be accepted if the entire remaining capacity of the knapsack (all remaining resources) were to be used only for that SP. The algorithm starts with the feasible solution $(n_p = 0)_{p=1..P}$, i.e., 0 users for each SP. At each iteration, it selects the SP that generates the highest total reward with its effective capacity, and commits a proportion, say $\alpha$, of its effective capacity to that SP. As such, this algorithm always generates a feasible solution in each iteration. In essence, this method uses a ``max-min'' criterion to make variable selection decisions and reflects the multidimensional nature of the general MDKP. In addition, it depletes the effective capacity at a geometric rate $\alpha$ and in the meantime avoids creating \emph{bottleneck} conditions for other SPs. The ability of this method to generate a
feasible solution and to include multiple users of the selected SP in the solution in each iteration results in superior computational efficiency over other heuristic methods. 

\begin{algorithm}[hbt!]
\caption{Primal Heuristic Algorithm}
\label{alg:heuristic}
\KwData{$n \geq 0$}
\KwResult{$\boldsymbol{n^*}$}
$n_p \gets 0, p = 1 \cdots P$\;
$E \gets \{p | n_p = 0 \} $\;
$\bar{K^r} \gets K^r, \forall r \in \mathcal{R} $\;
$\bar{N_p} \gets N_p, p = 1 \cdots P$\;

$\bar{C_p} \gets \min_r  \floor* {\{\frac{\bar{K^r}}{z^r_p}\}}, p = 1 \cdots P $\;

\While{$ \exists p,  \bar{C_p} \neq 0$}
{$R_p \gets \xi_p \times \bar{C_p}, \forall p$\;
      $p^* \gets \arg \max_p \{R_p\}$\;
      $I_{p^*} \gets \min(\bar{N_{p^*}}, \max(1, \floor* {\alpha \bar{C_{p^*}}}))$\;
      $n_{p^*} \gets n_{p^*} + I_{p^*} $\;
      $\bar{K^r} \gets \bar{K^r} - z_{p^*}^r \times I_{p^*}, \forall r \in \mathcal{R} $\;
      $\bar{N_{p^*}} \gets \bar{N_{p^*}} - I_{p^*}$\;
      \If{$\bar{N_{p^*}} = 0 \textbf{ or } \alpha = 1$}{$E \gets E - \{p^*\} $\;}{}
      \If{$E = \emptyset $}{$break$\;}
    }
    $\boldsymbol{n^*} \gets (n_p)_{p = 1 \cdots P}$\;
\end{algorithm}

The greediness of Algorithm~\ref{alg:heuristic} is determined by the selection of the greedy coefficient $\alpha$. As $\alpha$ increases, the rate at which the available resources are consumed by the selected SP in each iteration increases. In the extreme case, $\alpha = 1$  , the selected SP can use its maximal effective capacity and thus maximum feasible number of users will be included to the solution in a single
iteration. For small $\alpha$, the algorithm becomes conservative in its resource commitment to the selected SP.
The algorithm might even accept only a single user of a SP in an iteration as
the resource capacities become tight. The use of the greedy coefficient reduces the possibility of creating bottleneck conditions for certain constraints, which may result in reduced rewards in future iterations. Moreover, the heuristic is likely to select different items in consecutive iterations since the maximum rewards may change over time.
\end{comment}


==> todo.tex <==
- Why do we use the streaming algorithm? Computing the optimal value has scalability problems?
- Let's add the wifi-5G-resource block in the resource pool (we thus have 3 resource types), otherwise we are actually only allocating CPU
- Let's plot actual average delay instead of f.
- We cannot simply use formulation of [1] as multiple resources are more complicated.
[1] Chu, W., Dehghan, M., Lui, J. C. S., Towsley, D., & Zhang, Z. L. (2018). Joint cache resource allocation and request routing for in-network caching services. Computer Networks, 131, 1–14. https://doi.org/10.1016/j.comnet.2017.11.009
